Interference, Bias, and Variance in Two-Sided Marketplace Experimentation: Guidance for Platforms

Two-sided marketplace platforms often run experiments to test the effect of an intervention before launching it platform-wide. A typical approach is to randomize individuals into the treatment group, which receives the intervention, and the control group, which does not. The platform then compares the performance in the two groups to estimate the effect if the intervention were launched to everyone. We focus on two common experiment types, where the platform randomizes individuals either on the supply side or on the demand side. The resulting estimates of the treatment effect in these experiments are typically biased: because individuals in the market compete with each other, individuals in the treatment group affect those in the control group and vice versa, creating interference. We develop a simple tractable market model to study bias and variance in these experiments with interference. We focus on two choices available to the platform: (1) Which side of the platform should it randomize on (supply or demand)? (2) What proportion of individuals should be allocated to treatment? We find that both choices affect the bias and variance of the resulting estimators but in different ways. The bias-optimal choice of experiment type depends on the relative amounts of supply and demand in the market, and we discuss how a platform can use market data to select the experiment type. Importantly, we find in many circumstances, choosing the bias-optimal experiment type has little effect on variance. On the other hand, the choice of treatment proportion can induce a bias-variance tradeoff, where the bias-minimizing proportion increases variance. We discuss how a platform can navigate this tradeoff and best choose the treatment proportion, using a combination of modeling as well as contextual knowledge about the market, the risk of the intervention, and reasonable effect sizes of the intervention.

==> optimizing_design.tex <==
\section{Optimizing experiments: Experiment type}

In this section we study two levers that a platform has for bias minimization: the choice of experiment type ($\CR$ or $\LR$) and the treatment allocation for a given experiment type ($a_C$ and $a_L$). We analyze the bias in a large market as $N \to \infty$. 

For some (but not all) interventions, the platform can choose whether to run a $\CR$ or $\LR$ experiment. Consider an intervention that provides further information on a listing, perhaps by giving a lengthier description. This intervention could be tested through either a $\CR$ or $\LR$ experiment. In a $\CR$ experiment, customers would be randomized into treatment and control;  treatment customers would see listings with lengthier descriptions and control customers would see listings with the original descriptions. In an $\LR$ experiment, listings would be randomized into treatment and control; all customers would see treatment listings with lengthier descriptions and control listings with the original descriptions. 

This choice of $\CR$ and $\LR$ is not always available, however. In the previous example, perhaps the difference between the two description versions is so stark that running an $\LR$ design and thus showing a given customer both the original and extended descriptions would create a disruptive customer experience, leaving $\CR$ as the only option. In another example, suppose that the platform is testing a price reduction but for legal reasons is unable to show different customers different prices for a given listing. In such a scenario, $\LR$ is the only valid design. There may be a number of such reasons why a platform is constrained to using a single design, either $\LR$ or $\CR$. 

Thus in some scenarios, the platform can choose both the experiment type and treatment allocation and in other scenarios the platform can only choose the treatment allocation, with the type of experiment fixed. We thus consider how to minimize bias in both types of scenarios. 


\input{optimizing_exp_type}




\input{optimizing_allocation}



\subsection{Comparison of experiment type and treatment allocation.}


\begin{figure}
    \centering
    \includegraphics[scale=0.6]{figures/range_cr_lr_bias_m2e20_n2e16-2e24_heterogen_mult.png}
    \caption{\todo{}}
    \label{fig:design_and_allocation_varying_lambda}
\end{figure}


==> optimizing_design_old.tex <==
\section{Optimizing platform experiments}
\label{sec:optimizing_experiments}

We utilize the structural results from Section \ref{sec:Asymptotic_results} to optimize experiments with respect to bias and variance. Whereas in Section \ref{ssec:limiting_lr_cr_bias} we studied the factors that influence bias that are out of the platform's (immediate) control, here we focus on the aspects of experimental design that the platform \textit{can} control, namely the type of experiment run ($\CR$ or $\LR$) and the proportion allocated to treatment ($a_C$ and $a_L$, respectively). Section \ref{sec:optimizing_experiments} largely explores these design choices through theory and simulations and Section \ref{} will discuss the practical implications for platforms running these experiments. 

We first consider bias minimization in Section \ref{ssec:bias_minimization} and analyze two decisions: the type of the experiment run and the treatment allocation. We discuss both the feasibility of these two decisions as well as their effects on the resulting bias of an experiment. For the choice between $\LR$ and $\CR$, we show that the relative bias of $\CR$ and $\LR$ experiments is largely driven by by relative demand $\lambda$ on the platform. Once the experiment type is fixed, the platform must choose the treatment allocation. This allocation is typically chosen for convenience reasons but we show that, perhaps surprisingly, the fraction allocated to treatment affects the bias of an experiment \gw{This sentence is confusing. In reality, this is typically 50/50 due to power considerations, except if there are practical considerations not to treat 50\% (e.g., too risky, too expensive)}. In many settings, the bias-optimal treatment allocation lies at an endpoint of the range $[0,1]$. We then compare the relative importance of optimizing the experiment type versus optimizing the treatment allocation. 
\hl{Update once we have plot.}

In Section \ref{ssec:variance_optimization} we consider variance minimization and show that the variance minimizing designs for both $\CR$ and $\LR$ lie near $a_C=0.5$ and $a_L=0.5$, respectively, though the exact optimal point may depend on market parameters. In particular, the variance minimizing design differs from the bias minimizing design, thus inducing a bias-variance tradeoff. We use simulations to explore the tradeoff and find the optimal design when jointly optimizing for bias and variance; the optimal solution here is more complicated and depends on several market characteristics. Section \ref{} will provide heuristics for how a platform can navigate this bias-variance tradeoff in practice.


\subsection{Bias minimization}
\label{ssec:bias_minimization}
In this section we study two levers that a platform has for bias minimization: the choice of experiment type ($\CR$ or $\LR$) and the treatment allocation for a given experiment type ($a_C$ and $a_L$). We analyze the bias in a large market as $N \to \infty$. 

For some (but not all) interventions, the platform can choose whether to run a $\CR$ or $\LR$ experiment. Consider an intervention that provides further information on a listing, perhaps by giving a lengthier description. This intervention could be tested through either a $\CR$ or $\LR$ experiment. In a $\CR$ experiment, customers would be randomized into treatment and control;  treatment customers would see listings with lengthier descriptions and control customers would see listings with the original descriptions. In an $\LR$ experiment, listings would be randomized into treatment and control; all customers would see treatment listings with lengthier descriptions and control listings with the original descriptions. 

This choice of $\CR$ and $\LR$ is not always available, however. In the previous example, perhaps the difference between the two description versions is so stark that running an $\LR$ design and thus showing a given customer both the original and extended descriptions would create a disruptive customer experience, leaving $\CR$ as the only option. In another example, suppose that the platform is testing a price reduction but for legal reasons is unable to show different customers different prices for a given listing. In such a scenario, $\LR$ is the only valid design. There may be a number of such reasons why a platform is constrained to using a single design, either $\LR$ or $\CR$. 

Thus in some scenarios, the platform can choose both the experiment type and treatment allocation and in other scenarios the platform can only choose the treatment allocation, with the type of experiment fixed. We thus consider how to minimize bias in both types of scenarios. 


\subsubsection{Optimizing treatment allocation in a $\CR$ experiment.}
\label{sssec:optimizing_treat_allocation}

Consider the case where the experiment type is fixed and the platform must choose the treatment allocation. We start with this problem because it is a subproblem of the decision that a platform makes when controlling both the design and treatment allocation. 

We consider the bias in a large market setting as $N \to \infty$. 
For a $\CR$ design with treatment probability $a_C$, define the asymptotic bias of the experiment to be $B_\CR(a_C)$ where 
$$B_\CR(a_C) = \lim_{N \rightarrow \infty} N^{-1}\left( \E[\widehat{\GTE}_\CR^{(N)}(a_C)] - \GTE^{(N)} \right).$$

Similarly, for a $\LR$ design with treatment probability $a_L$, define the asymptotic bias to be 
$B_\LR(a_L)$ where 
$$B_\LR(a_L) = \lim_{N \rightarrow \infty} N^{-1}\left( \E[\widehat{\GTE}_\LR^{(N)}(a_L)] - \GTE^{(N)} \right).$$


First and foremost, we show that the treatment allocation affects the resulting bias of an experiment. Secondly, the bias-minimizing treatment allocation probability often lies at an endpoint of the range $[0,1]$, for both $\CR$ and $\LR$. 

Recall that we call an intervention \textit{multiplicative} if there exists an $\alpha$ such that $\tilde{\Phi} = \alpha \Phi$. That is, the intervention has the same multiplicative lift on the consideration probability across all customer and listing types. The following result shows that for $\CR$ and a multiplicative intervention, the bias is decreasing in $a_C$ if $\alpha>0$ and increasing in $a_C$ if $\alpha>0$.




\begin{theorem}
\label{Thm_opt_bias_ac}
\newhl{Suppose that the intervention is multiplicative on $\Phi$ with parameter $\alpha$. If $\alpha>1$, then the asymptotic bias of the $\CR$ estimator decreases as $a_C$ increases. If $\alpha<1$, then the asymptotic bias of the $\CR$ estimator increases as $a_C$ increases. }
\end{theorem}
\begin{proof}
\newhl{We prove the result in the case where $\alpha>1$. The case where $\alpha<1$ holds by symmetry.}
By Lemma~\ref{Lemma_upward_bias}, we know the asymptotic bias of the $\CR$ estimator is positive for any fixed choice of $a_C\in(0,1)$ when the intervention is positive and multiplicative on $\Phi$. Thus, minimizing the asymptotic bias is equivalent to minimizing the limit of the expectation of $\gtehatcr$, given in Proposition~\ref{Prop_limit_estimator_expectation} as
\[
    E_{\CR}(a_C) := \lambda \sum_{\tinT} \rho(\theta) \bsigma \cdot \left(\tilde{\bPhi}_{app}(\cdot,\theta) - \bm{\Phi}_{app}(\cdot,\theta)\right) F\left(\lambda \bsigma \cdot \left(a_C \tilde{\bPhi}_{app}(\cdot,\theta) + (1-a_C) \bm{\Phi}_{app}(\cdot,\theta)\right)\right).
\]
Taking partial derivative with respect to $a_C$, we find
\begin{equation}\label{Eqn_partial_derivative_ac:Thm_opt_bias_ac}
    \frac{\partial}{\partial a_C} E_{\CR}(a_C) = \lambda^2 \sum_{\tinT} \rho(\theta) \left(\bsigma \cdot \left(\tilde{\bPhi}_{app}(\cdot,\theta) - \bm{\Phi}_{app}(\cdot,\theta)\right)\right)^2 F'\left(A\right),
\end{equation}
where $A$ is the short-hand for the argument in $F(\cdot)$ above. This value is strictly negative since $F'(a) < 0$ for any $a\in\R^+$. Thus, $E_{\CR}(a_C)$ is strictly decreasing in $a_C$, and so is the asymptotic CR bias.
\end{proof}





\hl{Add intuition here about marginal customer. 1) GTE>0. 2) Estimate > GTE. Marginal customer minimizes estimate if assigned to treatment. }

We conjecture that a more general result than Theorem \ref{Thm_opt_bias_ac} holds for a class of interventions beyond multiplicative interventions, as long as the heterogeneity across in the  lifts $\tilde{\conprob}(\gamma, \theta) - \conprob(\gamma, \theta)$ is sufficiently small across pairs of $\gamma$ and $\theta$. On this class of interventions, we conjecture that if the $\GTE>0$, then the asymptotic bias of $\CR$ is decreasing in $a_C$ and if the $\GTE<0$, the asymptotic bias is increasing in $a_C$. Note that in case of the multiplicative intervention, when $\GTE>0$ whenever $\alpha>1$ and so Theorem \ref{Thm_opt_bias_ac} is a special case of this broader conjecture.

To see two examples of where this conjecture fails, we show two scenarios in a heterogeneous market place with listing types $\theta_1$ and $\theta_2$ and a single customer type $\gamma$. In the first example, the intervention decreases $\conprob(\gamma, \theta_1)$ and increases $\conprob(\gamma, \theta_2)$. In the second, the intervention increases both $\conprob(\gamma, \theta_1)$ and $\conprob(\gamma, \theta_2)$ but increases one by a much larger margin.
\todo{Add plots of $\CR$ bias in both of these scenarios. Describe actual parameters. } \gw{Perhaps worth mentioning that conjecture fails, but not sure whether worth adding these examples. }


Though the treatment allocation $a_C$ affects the magnitude of the bias in a $\CR$ experiment, we can show that the choice of $a_C$ does not affect the bias too much. More specifically, bound the maximum difference in bias with respect to the choice of $a_C$. 

For a $\CR$ experiment, we call the difference between the highest possible and lowest possible bias attained by varying $a_C$
$$\sup_{a_C\in(0,1)} B(a_C) - \inf_{a_C\in(0,1)} B(a_C)$$ the \textit{$\CR$ bias differential} in $a_C$. 


\begin{corollary}
Consider a $\CR$ experiment. The bias differential is bounded by
\[
    \sup_{a_C\in(0,1)} B(a_C) - \inf_{a_C\in(0,1)} B(a_C) \leq \lambda^2 \left( \sup_{\ginG,\tinT} \tilde{\phi}_{con}(\gamma,\theta)-\phi_{con}(\gamma,\theta)\right)^2,
\]
\end{corollary}
\begin{proof}
This is a direct consequence of \eqref{Eqn_partial_derivative_ac:Thm_opt_bias_ac}, which implies that $E_{\CR}$ has Lipshitz coefficient
\[
    \lambda^2 \left( \sup_{\ginG,\tinT} \tilde{\phi}_{con}(\gamma,\theta)-\phi_{con}(\gamma,\theta)\right)^2.
\]
\end{proof}
Note that this result holds for any intervention, even when the intervention is not multiplicative on $\Phi$.

This bound depends on the relative demand $\lambda$ as well as the size of the lift that the intervention has on the consideration probabilities.

\hl{TODO. Plot 1. Fix $\alpha$ and vary $\lambda$. Plot bias differential as $\lambda$ changes. Plot the bound you derived on the same axis.}

\hl{TODO. Plot 2. Fix $\lambda$. Plot bias differential and bound as $\alpha$ changes. Plot your bound as well. }

\subsubsection{Optimizing treatment allocation in an $\LR$ experiment.}
We similarly show that for the $\LR$ design, the bias is monotonically changing in $a_L$. However, the result here is more subtle: for a fixed intervention, the bias may be monotonically increasing or monotonically decreasing in $a_L$, depending on both the sign of the change in the consideration probability and the relative demand $\lambda$. 

We prove this result for a homogeneous market (where trivially the intervention is multiplicative).  We conjecture that a more general statement holds for multiplicative interventions in a heterogeneous market as well, and also for interventions where the lifts on the consideration probabilities $\conprob(\gamma, \theta)$ are not ``too" heterogeneous across $\gamma$ and $\theta$. 
\begin{theorem}
Consider a homogeneous market (with only one type of listings and customers), where the consideration probability changes from $\conprob$ to $\tilde{\conprob}$. Then the asymptotic bias of the LR estimator, as a function of $a_L$, has no local minimum inside $(0,1)$. In other words, it achieves infimum either as $a_L\to 0$ or as $a_L\to 1$. \newhl{Furthermore, there exists a $\lambda^*$ such that 
\begin{enumerate}[label=\alph*)]
    \item If $\tilde{\conprob}>\conprob$, then  $B_\LR(a_L)$ is decreasing in $a_L$ for $\lambda < \lambda^*$ and  $B_\LR(a_L)$ is increasing in $a_L$ for $\lambda>\lambda^*$ . 
    \item If $\tilde{\conprob}<\conprob$, then $B_\LR(a_L)$ is increasing in $a_L$ for $\lambda < \lambda^*$  and $B_\LR(a_L)$ is decreasing in $a_L$ for $\lambda>\lambda^*$.
\end{enumerate}}
\gz{TODO: Does this hold for heterogeneous case? Can we identify the change point (right now given by an implicit function)?}
\end{theorem}
\begin{proof}
\gz{TODO}
\end{proof}

More specifically, we conjecture that on a broader class of interventions, there exists a cutoff $\lambda^*$ such that when the $\GTE>0$, the $\LR$ asymptotic bias is decreasing in $a_L$ for $\lambda<\lambda^*$ and increasing in $a_L$ for $\lambda>\lambda^*$, and vice versa for $\GTE<0$. 

\hl{TODO. Plots that support conjecture in heterogeneous multiplicative case.}

\hl{Do we have a counterexample with an interior optimal point for a non-multiplicative scenario?}

\gw{Do we have any intuition here?}

\subsubsection{Optimizing experiment type.}



Using Lemma \ref{Lemma_limit_estimator_expectation}, we can explicitly derive the dependence of the $\CR$ and $\LR$ bias as a function of the relative demand, customer and listing type distributions, and pre-treatment and post-treatment consideration probabilities.  In particular, we can show that the $\CR$ estimator becomes unbiased as the relative demand diminishes and the $\LR$ estimator becomes unbiased as the relative demand increases. 


\gw{This is a central result. Seems to come too late to me. Personally, I would flip the order with opt of allocation.}

\begin{theorem}[Unbiasedness in market extremes]
\hl{Perhaps move to Section 3?}

\todo{Figure out what normalization we need here. $\min\{\lambda, 1\}$?}
\todo{Add statement that the other design is biased. }
\begin{enumerate}
    \item Consider a sequence of markets where $\lambda \to 0$. Along this sequence, for any $a_C \in (0,1)$ we have $\gtehatcr(a_C)-\GTE \to 0$. That is, the $\CR$ asymptotic bias approaches 0 as the relative demand decreases. 
    \item Consider a sequence of markets where $\lambda \to \infty$. Along this sequence, for any $a_L \in (0,1)$ we have $\gtehatlr(a_C) - \GTE \to 0$. That is, the $\LR$ asymptotic bias approaches 0 as the relative demand increases. 
\end{enumerate}
\end{theorem}
\begin{proof}
\todo{}
\end{proof}

Intuitively, $\CR$ bias arises when treatment and control customers apply to the same listing and thus compete with each other. $\LR$ bias arises when customers consider both control and treatment listings in their consideration set, creating competition between listings and changing the probability a given listing receives an application. In a demand constrained market as $\lambda \to 0$, there are few enough customers that customers are unlikely to apply to the same listings and so the $\CR$ estimate is unbiased. However, the existing customers will still have multiple listings in their consideration sets, so in an $\LR$ experiment, treatment and control listings will still compete and the $\LR$ estimate will be biased.

In over-demanded market as $\lambda \to \infty$, many customers will apply to a given listing, creating competition between customers and a bias in the $\CR$ estimate. However, as the number of customers grows, all listings will receive an application (and thus be booked), regardless of the competition created by multiple listings appearing in a customer's consideration set. Thus the $\LR$ estimate becomes unbiased. 
\hl{Is intuition for why $\LR$ is unbiased different in this model? ie unbiased because everything is booked in the one-shot model?}

\subsubsection{Optimizing both experiment type and treatment allocation.}
It is then natural to ask how the platform can optimize both levers

\begin{figure}
    \centering
    \includegraphics[scale=0.6]{figures/range_cr_lr_bias_m2e20_n2e16-2e24_heterogen_mult.png}
    \caption{\todo{}}
    \label{fig:design_and_allocation_varying_lambda}
\end{figure}


\subsection{Variance minimization}
\label{ssec:variance_optimization}
